The Dust-Selected Molecular Clouds in the Northeast Region of the Small Magellanic Cloud

We present a high-sensitivity ($1\sigma<1.6~\mathrm{mJy~beam^{-1}}$) continuum observation in a 343 arcmin$^2$ area of the northeast region in the Small Magellanic Cloud at a wavelength of 1.1 mm, conducted using the AzTEC instrument on the ASTE telescope. In the observed region, we identified 20 objects by contouring $10\sigma$ emission. Through spectral energy distribution (SED) analysis using 1.1 mm, $Herschel$, and $Spitzer$ data, we estimated the gas masses of $5\times 10^3-7\times 10^4~\mathrm{M_\odot}$, assuming a gas-to-dust ratio of 1000. Dust temperature and the index of emissivity were also estimated as $18-33$ K and $0.9-1.9$, respectively, which are consistent with previous low resolution studies. The relation between dust temperature and the index of emissivity shows a weak negative linear correlation. We also investigated five CO-detected dust-selected clouds in detail. The total gas masses were comparable to those estimated from the Mopra CO data, indicating that the assumed gas-to-dust ratio of 1000 and the $X_\mathrm{CO}$ factor of $1\times10^{21}~\mathrm{cm^{-2}~(K~km~s^{-1})^{-1}}$, with uncertainties of a factor of 2, are reliable for the estimation of the gas masses of molecular or dust-selected clouds. Dust column density showed good spatial correlation with CO emission, except for an object that associates with bright young stellar objects. The $8~\mathrm{\mu m}$ filamentary and clumpy structures also showed similar spatial distribution with the CO emission and dust column density, supporting the fact that polycyclic aromatic hydrocarbon emissions arise from the surfaces of dense gas and dust clouds.

==> dust-selected-molecular (12)/table1.tex <==
\begin{deluxetable*}{rcccccccc}
\tabletypesize{\scriptsize}
\tablecaption{AzTEC/ASTE 1.1 mm extended source catalog of the SMC NE region. \label{table:catalog_fruit}}
\tablehead{Object ID&$\alpha$&$\delta$&1.1mm Peak flux&S/N&1.1 mm total flux&$R$&Star formation?&Map edge?\\
&$(J2000)$&$(J2000)$&(mJy~beam$^{-1}$)&&(mJy)&(pc)}
\startdata
NEdeep-1&00$^h$58$^m$45.9$^s$&-72$^\circ$13$'$18$''$&48.7 $\pm$2.3 &21.0 &28.8 $\pm$4.1 &8.0 &Yes&Yes\\
2&00$^h$57$^m$30.7$^s$&-72$^\circ$32$'$30$''$&34.1 $\pm$1.3 &27.2 &42.5 $\pm$5.5 &10.2 &Yes&No\\
3&00$^h$58$^m$31.5$^s$&-72$^\circ$15$'$12$''$&31.6 $\pm$1.5 &21.5 &191.1 $\pm$24.5 &22.9 &No&No\\
4&00$^h$56$^m$42.0$^s$&-72$^\circ$23$'$29$''$&24.4 $\pm$1.2 &20.2 &142.0 $\pm$18.2 &20.0 &Yes&No\\
5&00$^h$56$^m$46.1$^s$&-72$^\circ$21$'$05$''$&21.9 $\pm$1.2 &18.0 &27.1 $\pm$3.6 &9.2 &Yes&No\\
6&00$^h$58$^m$38.8$^s$&-72$^\circ$35$'$00$''$&21.5 $\pm$2.2 &9.6 &10.4 $\pm$2.6 &5.8 &No&Yes\\
7&00$^h$58$^m$41.1$^s$&-72$^\circ$27$'$18$''$&21.3 $\pm$1.2 &17.6 &19.3 $\pm$2.6 &7.6 &Yes&No\\
8&00$^h$56$^m$54.3$^s$&-72$^\circ$16$'$35$''$&21.2 $\pm$1.7 &12.5 &156.6 $\pm$20.1 &22.6 &Yes&Yes\\
9&00$^h$58$^m$17.3$^s$&-72$^\circ$28$'$18$''$&18.6 $\pm$1.2 &15.0 &11.6 $\pm$1.9 &6.1 &No&No\\
10&00$^h$55$^m$59.9$^s$&-72$^\circ$21$'$34$''$&18.3 $\pm$1.3 &13.8 &12.3 $\pm$2.0 &6.2 &No&No\\
11&00$^h$58$^m$58.1$^s$&-72$^\circ$21$'$59$''$&17.4 $\pm$1.2 &14.3 &20.1 $\pm$2.7 &8.3 &No&No\\
12&00$^h$56$^m$12.9$^s$&-72$^\circ$23$'$46$''$&17.1 $\pm$1.2 &13.9 &12.7 $\pm$2.0 &6.5 &No&No\\
13&00$^h$58$^m$17.3$^s$&-72$^\circ$30$'$18$''$&16.9 $\pm$1.3 &13.4 &16.7 $\pm$2.3 &7.6 &No&No\\
14&00$^h$56$^m$49.5$^s$&-72$^\circ$30$'$23$''$&16.6 $\pm$1.3 &13.1 &14.4 $\pm$2.1 &7.1 &No&No\\
15&00$^h$56$^m$07.1$^s$&-72$^\circ$28$'$22$''$&16.6 $\pm$1.3 &12.4 &7.6 $\pm$1.8 &5.0 &Yes&No\\
16&00$^h$56$^m$03.6$^s$&-72$^\circ$23$'$46$''$&16.0 $\pm$1.2 &12.8 &10.2 $\pm$1.8 &5.9 &No&No\\
17&00$^h$56$^m$05.2$^s$&-72$^\circ$20$'$52$''$&15.9 $\pm$1.3 &11.9 &$<$4.9 $\pm$2.0 &4.1 &No&No\\
18&00$^h$56$^m$26.1$^s$&-72$^\circ$23$'$29$''$&15.8 $\pm$1.2 &13.0 &7.7 $\pm$1.7 &5.1 &Yes&No\\
19&00$^h$56$^m$00.1$^s$&-72$^\circ$19$'$58$''$&15.4 $\pm$1.4 &10.8 &14.8 $\pm$2.2 &7.2 &No&No\\
20&00$^h$58$^m$07.9$^s$&-72$^\circ$23$'$06$''$&15.0 $\pm$1.2 &12.6 &$<$5.0 $\pm$1.8 &4.2 &No&No\\
\enddata
\tablecomments{The columns give (1) source ID, (2) right ascension, (3) declination, (4) observed peak flux and noise level at 1.1 mm, (5) signal-to-noise ratio, (6) 1.1 mm total flux, (7) source radius, (8) whether the object associates with YSOs or $24~\micron$ objects, and (9) whether the object is located at the map edge or not.}
\end{deluxetable*}



==> dust-selected-molecular (12)/table2.tex <==
\begin{deluxetable*}{rccccccccc}
\tabletypesize{\scriptsize}
\rotate
\tablewidth{22cm}
\tablecaption{Total flux densities of the 1.1 mm extended objects. \label{table:sed}}
\tablehead{Object ID&$S_\mathrm{1.1mm}$&$S_\mathrm{{\it Herschel} 500\mu m}$&$S_\mathrm{{\it Herschel} 350\mu m}$&$S_\mathrm{{\it Herschel} 250\mu m}$&$S_\mathrm{{\it Herschel} 160\mu m}$&$S_\mathrm{{\it Herschel} 100\mu m}$&$S_\mathrm{{\it Spitzer} 70\mu m}$&$S_\mathrm{{\it Spitzer} 24\mu m}$\\
&(mJy)&(mJy)&(mJy)&(mJy)&(mJy)&(mJy)&(mJy)&(mJy)}
\startdata
NEdeep-1 &  28.77  $\pm$ 4.05  &  219.57  $\pm$ 29.21  & 499.99  $\pm$ 42.50  &  865.16  $\pm$ 74.42  &  1348.15  $\pm$ 209.14  & $<$ 880.38  $+$ 294.55  & $<$ 3429.12  $+$ 172.15  & $<$ 117.67  $+$ 5.06  \\
2 &  42.50  $\pm$ 5.49  &  458.14  $\pm$ 58.91  & 1133.80  $\pm$ 145.45  &  2396.13  $\pm$ 307.31  &  5457.49  $\pm$ 781.40  &  7256.19  $\pm$ 1049.08  & $<$ 5666.17  $+$ 283.57  & $<$ 584.42  $+$ 23.42  \\
3 &  191.15  $\pm$ 24.48  &  1290.85  $\pm$ 165.33  & 2804.53  $\pm$ 224.40  &  4315.19  $\pm$ 345.31  &  5355.56  $\pm$ 538.37  &  1929.04  $\pm$ 216.38  & $<$ 14249.72  $+$ 712.51  & $<$ 393.60  $+$ 15.76  \\
4 &  142.01  $\pm$ 18.19  &  1233.59  $\pm$ 158.00  & 2746.50  $\pm$ 219.76  &  5144.05  $\pm$ 411.61  &  8448.07  $\pm$ 847.12  &  6929.23  $\pm$ 701.90  & $<$ 7295.19  $+$ 364.81  & $<$ 186.96  $+$ 7.52  \\
5 &  27.14  $\pm$ 3.56  &  313.51  $\pm$ 40.57  & 735.53  $\pm$ 59.61  &  1442.02  $\pm$ 116.86  &  2785.09  $\pm$ 310.21  &  1846.36  $\pm$ 306.06  & $<$ 1739.19  $+$ 88.00  & $<$ 59.43  $+$ 2.88  \\
6 &  10.37  $\pm$ 2.60  &  76.10  $\pm$ 14.50  & 172.45  $\pm$ 23.76  &  326.48  $\pm$ 45.17  & $<$ 564.61  $+$ 226.32  & $<$ 503.26  $+$ 389.14  & $<$ 595.94  $+$ 36.61  & $<$ 12.50  $+$ 2.61  \\
7 &  19.29  $\pm$ 2.64  &  244.03  $\pm$ 32.04  & 635.78  $\pm$ 52.16  &  1433.03  $\pm$ 116.86  &  3179.00  $\pm$ 358.57  &  4056.86  $\pm$ 502.43  & $<$ 3113.91  $+$ 156.56  & $<$ 1232.81  $+$ 49.35  \\
8 &  156.64  $\pm$ 20.06  &  1205.48  $\pm$ 154.40  & 2654.83  $\pm$ 212.43  &  4927.65  $\pm$ 394.30  &  8909.95  $\pm$ 892.75  &  7685.05  $\pm$ 774.90  & $<$ 9161.29  $+$ 458.10  & $<$ 223.78  $+$ 8.98  \\
9 &  11.58  $\pm$ 1.90  &  141.30  $\pm$ 20.15  & 314.92  $\pm$ 29.08  &  569.66  $\pm$ 53.67  &  948.30  $\pm$ 227.46  & $<$ 650.74  $+$ 375.03  & $<$ 635.30  $+$ 37.76  & $<$ 19.94  $+$ 2.58  \\
10 &  12.29  $\pm$ 2.00  &  96.39  $\pm$ 15.13  & 185.58  $\pm$ 20.72  &  316.58  $\pm$ 37.88  & $<$ 480.18  $+$ 207.40  & $<$ 597.94  $+$ 364.99  & $<$ 695.84  $+$ 40.08  & $<$ 14.18  $+$ 2.46  \\
11 &  20.06  $\pm$ 2.71  &  180.47  $\pm$ 24.00  & 361.14  $\pm$ 30.77  &  580.18  $\pm$ 50.81  &  750.48  $\pm$ 168.82  & $<$ 577.87  $+$ 276.31  & $<$ 923.12  $+$ 48.51  & $<$ 17.41  $+$ 1.93  \\
12 &  12.67  $\pm$ 1.96  &  81.42  $\pm$ 13.34  & 192.31  $\pm$ 20.55  &  355.29  $\pm$ 38.94  &  766.82  $\pm$ 208.93  & $<$ 517.02  $+$ 351.03  & $<$ 734.78  $+$ 41.45  & $<$ 15.37  $+$ 2.39  \\
13 &  16.67  $\pm$ 2.34  &  193.16  $\pm$ 25.74  & 466.69  $\pm$ 39.13  &  893.76  $\pm$ 75.06  &  1612.17  $\pm$ 231.38  &  1064.76  $\pm$ 314.97  & $<$ 884.74  $+$ 47.17  & $<$ 26.68  $+$ 2.24  \\
14 &  14.44  $\pm$ 2.12  &  133.41  $\pm$ 18.70  & 284.63  $\pm$ 25.97  &  524.53  $\pm$ 48.53  &  910.94  $\pm$ 198.90  & $<$ 835.20  $+$ 326.61  & $<$ 903.96  $+$ 48.45  & $<$ 19.09  $+$ 2.23  \\
15 &  7.59  $\pm$ 1.83  &  62.01  $\pm$ 13.45  & 128.06  $\pm$ 20.69  &  227.14  $\pm$ 39.44  & $<$ 321.88  $+$ 252.35  & $<$ 296.14  $+$ 447.59  & $<$ 341.51  $+$ 30.01  & $<$ 32.78  $+$ 3.24  \\
16 &  10.19  $\pm$ 1.79  &  76.26  $\pm$ 13.36  & 166.25  $\pm$ 20.01  &  302.98  $\pm$ 37.95  & $<$ 600.05  $+$ 220.76  & $<$ 360.79  $+$ 381.19  & $<$ 589.28  $+$ 36.17  & $<$ 11.29  $+$ 2.56  \\
17 & $<$ 4.91  $+$ 2.02  & $<$ 31.78  $+$ 14.03  & 73.52  $\pm$ 22.99  & $<$ 133.06  $+$ 44.58  & $<$ 246.95  $+$ 310.52  & $<$ 265.75  $+$ 552.96  & $<$ 324.77  $+$ 34.57  & $<$ 6.95  $+$ 3.68  \\
18 &  7.68  $\pm$ 1.69  &  54.02  $\pm$ 12.56  & 127.18  $\pm$ 19.93  &  232.85  $\pm$ 38.32  & $<$ 503.19  $+$ 250.32  & $<$ 446.56  $+$ 440.42  & $<$ 466.29  $+$ 33.62  & $<$ 18.65  $+$ 3.00  \\
19 &  14.80  $\pm$ 2.22  &  160.25  $\pm$ 21.92  & 379.77  $\pm$ 32.98  &  741.74  $\pm$ 64.37  &  1578.41  $\pm$ 236.04  &  1417.27  $\pm$ 343.46  & $<$ 1262.21  $+$ 65.43  & $<$ 33.48  $+$ 2.47  \\
20 & $<$ 5.02  $+$ 1.79  &  67.04  $\pm$ 15.42  & 150.84  $\pm$ 24.14  &  284.33  $\pm$ 46.78  & $<$ 579.83  $+$ 305.80  & $<$ 482.72  $+$ 538.76  & $<$ 405.30  $+$ 35.92  & $<$ 7.53  $+$ 3.58  \\
\enddata
\tablecomments{Two values provided in each cell show the representative fluxes and $1\sigma$ errors. We shows the upper limit values for the combination of the uniform and normal distribution in the MCMC analysis as the sign of "$<$".}
\end{deluxetable*}

==> dust-selected-molecular (12)/table3.tex <==
\begin{deluxetable*}{rcccccc}
\tabletypesize{\scriptsize}
\tablewidth{12cm}
\tablecaption{Physical properties of the 1.1 mm extended objects. \label{table:sedfit}}
\tablehead{Object ID&$T_\mathrm{dust}$&$M_\mathrm{dust}$&$M_\mathrm{gas}$&$\beta$&$n_\mathrm{H_2}$&$N_\mathrm{H_2}$\\
&(K)&($\mathrm{M_\sun}$)&($\times 10^3 \mathrm{M_\sun}$)& &($\mathrm{H_2/cm^3}$)&($\mathrm{\times 10^{20} H_2/cm^2}$)}
\startdata
NEdeep-1&$24.3\pm2.3$&$<8.6$&$<8.6$&$1.06\pm0.14$&$<180.0$&$<59.2$\\
2&$33.0\pm2.3$&$10.7^{+2.8}_{-2.2}$&$10.7^{+2.8}_{-2.2}$&$1.24\pm0.11$&$35.7^{+9.3}_{-7.4}$&$15.0^{+3.9}_{-3.1}$\\
3&$19.5\pm0.7$&$70.4^{+14.1}_{-11.7}$&$70.4^{+14.1}_{-11.7}$&$1.12\pm0.11$&$21.0^{+4.2}_{-3.5}$&$19.8^{+4.0}_{-3.3}$\\
4&$26.3\pm1.3$&$35.2^{+7.2}_{-6.0}$&$35.2^{+7.2}_{-6.0}$&$1.09\pm0.10$&$15.7^{+3.2}_{-2.7}$&$12.9^{+2.6}_{-2.2}$\\
5&$23.4\pm1.2$&$16.3^{+3.7}_{-3.0}$&$16.3^{+3.7}_{-3.0}$&$1.47\pm0.11$&$75.1^{+17.2}_{-14.0}$&$28.4^{+6.5}_{-5.3}$\\
6&$25.2\pm5.5$&$<9.7$&$<9.7$&$1.12\pm0.31$&$<529.1$&$<126.8$\\
7&$30.1\pm1.8$&$8.4^{+1.9}_{-1.5}$&$8.4^{+1.9}_{-1.5}$&$1.46\pm0.10$&$69.6^{+15.6}_{-12.7}$&$21.7^{+4.9}_{-4.0}$\\
8&$29.1\pm1.6$&$25.1^{+5.3}_{-4.4}$&$25.1^{+5.3}_{-4.4}$&$0.93\pm0.10$&$7.8^{+1.7}_{-1.4}$&$7.2^{+1.5}_{-1.3}$\\
9&$20.7\pm2.7$&$<18.1$&$<18.1$&$1.54\pm0.19$&$<868.5$&$<216.9$\\
10&$23.6\pm5.1$&$<9.3$&$<9.3$&$1.00\pm0.24$&$<411.1$&$<105.3$\\
11&$20.1\pm2.5$&$<16.2$&$<16.2$&$1.22\pm0.18$&$<303.8$&$<103.7$\\
12&$30.8\pm3.6$&$<1.8$&$<1.8$&$0.86\pm0.13$&$<72.2$&$<19.2$\\
13&$22.8\pm1.6$&$11.0^{+3.3}_{-2.6}$&$11.0^{+3.3}_{-2.6}$&$1.49\pm0.13$&$91.1^{+27.7}_{-21.2}$&$28.4^{+8.6}_{-6.6}$\\
14&$26.0\pm3.7$&$<6.5$&$<6.5$&$1.12\pm0.17$&$<195.8$&$<57.2$\\
15&$22.3\pm4.6$&$<8.6$&$<8.6$&$1.17\pm0.27$&$<732.6$&$<151.3$\\
16&$25.8\pm4.6$&$<5.1$&$<5.1$&$1.01\pm0.20$&$<266.5$&$<64.8$\\
17&$17.6\pm4.5$&$<21.9$&$<21.9$&$1.88\pm0.57$&$<3516.3$&$<587.4$\\
18&$24.2\pm4.5$&$<6.0$&$<6.0$&$1.12\pm0.25$&$<477.4$&$<100.5$\\
19&$27.9\pm2.3$&$5.0^{+1.5}_{-1.2}$&$5.0^{+1.5}_{-1.2}$&$1.28\pm0.12$&$48.8^{+14.8}_{-11.3}$&$14.4^{+4.4}_{-3.3}$\\
20&$18.9\pm5.3$&$<55.2$&$<55.2$&$1.90\pm0.50$&$<8122.2$&$<1396.1$\\\tableline
\enddata
\tablecomments{The columns give (1) Source ID, (2) dust temperature, (3) total dust mass, (4) total gas mass, (5) index of emissivity (6) $\mathrm{H_2}$ density, and (7) $\mathrm{H_2}$ column density. The errors and upper limits are provided by 1$\sigma$ and 3$\sigma$, respectively. }
\end{deluxetable*}

==> dust-selected-molecular (12)/table4.tex <==
\begin{deluxetable}{lcc}
\tabletypesize{\scriptsize}
\tablewidth{11cm}
\tablecaption{Summary of physical properties between the SMC NEdeep and wide survey objects.\label{table4}}
\tablehead{&This study (NEdeep)&SMC wide survey}
\startdata
Cloud number&17&43\\
$T_\mathrm{dust}$ range&17.6--33.0~K&17--45~K\\
$T_\mathrm{dust}$ ave.$\pm$std.&24.3$\pm$4.4~K&28.7$\pm$4.4~K\\
$\beta$ range&0.9--1.9&1.2 (fixed) \\
$\beta$ ave.$\pm$std.&1.29$\pm$0.29&--\\
$M_\mathrm{gas}$ range&(5.0--70)$\times 10^3~\mathrm{M_\sun}$&(4.1--336)$\times 10^3~\mathrm{M_\sun}$\\
$M_\mathrm{gas}$ median&$11.0\times 10^3~\mathrm{M_\sun}$&$44.6\times 10^3~\mathrm{M_\sun}$\\
$R$ range &4--23~pc&6--40~pc\\
$R$ median&7.1~pc&11.8~pc\\
$\mathrm{H_2}$ density range&16--91~$\mathrm{cm^{-3}}$&17--171~$\mathrm{cm^{-3}}$\\
$\mathrm{H_2}$ density ave.$\pm$std. dev.&$49\pm 29~\mathrm{cm^{-3}}$&$68\pm 36~\mathrm{cm^{-3}}$\\
$\mathrm{H_2}$ column density range&(13--28)$\times 10^{20}~\mathrm{cm^{-2}}$&(10--44)$\times 10^{20}~\mathrm{cm^{-2}}$\\
$\mathrm{H_2}$ column density ave.$\pm$std. dev.&(20$\pm$6)$\times 10^{20}~\mathrm{cm^{-2}}$&(29$\pm$8)$\times 10^{20}~\mathrm{cm^{-2}}$\\
\enddata
\tablecomments{Upper limit values of $M_\mathrm{gas}$, $\mathrm{H_2}$ density, and $\mathrm{H_2}$ column density are excluded from the statistics.}
\end{deluxetable}

==> dust-selected-molecular (12)/table5.tex <==
\begin{deluxetable}{lcccc}
\tabletypesize{\scriptsize}
\tablewidth{12cm}
\tablecaption{Comparison of gas masses estimated from dust and CO.\label{table5}}
\tablehead{Object ID&$M_\mathrm{gas, dust}$&$M_\mathrm{gas, CO}$&$M_\mathrm{gas, dust}/M_\mathrm{gas, CO}$&$L_\mathrm{CO}$\\
&($10^3~\mathrm{M_\odot}$)&($10^3~\mathrm{M_\odot}$)&&($10^2~\mathrm{K~km~s^{-1}~pc^2}$)}
\startdata
NEdeep-4&$35.2^{+7.2}_{-6.0}$&$44.2\pm4.4$&0.80&$20.3\pm2.3$\\
NEdeep-5&$16.3^{+3.7}_{-3.0}$&$9.1\pm0.9$&1.79&$4.2\pm0.4$\\
NEdeep-7&$8.4^{+1.9}_{-1.5}$&$10.7\pm1.1$&0.79&$4.9\pm0.5$\\
NEdeep-9&$<18.1$&$6.7\pm0.7$&--&$3.1\pm0.3$\\
NEdeep-13&$11.0^{+3.3}_{-2.6}$&$8.4\pm0.8$&1.31&$3.9\pm0.4$\\
\enddata
\end{deluxetable}
